A Model-Constrained Discontinuous Galerkin Network (DGNet) for Compressible Euler Equations with Out-of-Distribution Generalization

Real-time accurate solutions of large-scale complex dynamical systems are critically needed for control, optimization, uncertainty quantification, and decision-making in practical engineering and science applications, particularly in digital twin contexts. In this work, we develop a model-constrained discontinuous Galerkin Network (DGNet) approach, a significant extension to our previous work [Model-constrained Tagent Slope Learning Approach for Dynamical Systems], for compressible Euler equations with out-of-distribution generalization. The core of DGNet is the synergy of several key strategies: (i) leveraging time integration schemes to capture temporal correlation and taking advantage of neural network speed for computation time reduction; (ii) employing a model-constrained approach to ensure the learned tangent slope satisfies governing equations; (iii) utilizing a GNN-inspired architecture where edges represent Riemann solver surrogate models and nodes represent volume integration correction surrogate models, enabling capturing discontinuity capability, aliasing error reduction, and mesh discretization generalizability; (iv) implementing the input normalization technique that allows surrogate models to generalize across different initial conditions, geometries, meshes, boundary conditions, and solution orders; and (v) incorporating a data randomization technique that not only implicitly promotes agreement between surrogate models and true numerical models up to second-order derivatives, ensuring long-term stability and prediction capacity, but also serves as a data generation engine during training, leading to enhanced generalization on unseen data. To validate the effectiveness, stability, and generalizability of our novel DGNet approach, we present comprehensive numerical results for 1D and 2D compressible Euler equation problems.

==> Figs/2D_Hypersonic/Relative_error_test_data_model1_mesh.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{darkgray176}{RGB}{176,176,176}
\definecolor{lightgray204}{RGB}{204,204,204}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=lightgray204
},
tick align=outside,
tick pos=left,
x grid style={darkgray176},
xlabel={time step \(\displaystyle n_t\), \(\displaystyle \Delta\)t = 5e-07},
xmin=0, xmax=3000,
xtick style={color=black},
y grid style={darkgray176},
ylabel={Relative \(\displaystyle L^2\)-Error},
ymin=-0.00932221040129662, ymax=0.2,
ytick style={color=black}
]
\addplot [semithick, black, mark=x, mark size=2.5, mark repeat=20, mark options={solid}]
table {%
0 0
20 0.00619501434266567
40 0.00982013903558254
60 0.0120285488665104
80 0.0133296055719256
100 0.014854378066957
120 0.017359584569931
140 0.0188360996544361
160 0.0214205011725426
180 0.0223114024847746
200 0.0253668334335089
220 0.0262557491660118
240 0.0281777735799551
260 0.0301908906549215
280 0.0308875627815723
300 0.0338013395667076
320 0.0356782227754593
340 0.0368887707591057
360 0.0401219055056572
380 0.042598020285368
400 0.0448698215186596
420 0.0480800978839397
440 0.0512813031673431
460 0.054208792746067
480 0.0569460764527321
500 0.0593377165496349
520 0.0613932237029076
540 0.063091479241848
560 0.0645144060254097
580 0.0659320503473282
600 0.0672717839479446
620 0.0682600066065788
640 0.0688118636608124
660 0.0691985785961151
680 0.0698937103152275
700 0.0706328898668289
720 0.0708915442228317
740 0.0708660557866096
760 0.0709256008267403
780 0.0713970437645912
800 0.0724749490618706
820 0.0735321938991547
840 0.0741143748164177
860 0.0745159909129143
880 0.0750828012824059
900 0.0760365724563599
920 0.0775407552719116
940 0.0791831538081169
960 0.0805807635188103
980 0.0816169530153275
1000 0.0826425850391388
1020 0.0839095935225487
1040 0.0855074375867844
1060 0.0873949155211449
1080 0.0893508046865463
1100 0.0910307988524437
1120 0.0923949480056763
1140 0.0935696959495544
1160 0.0948033630847931
1180 0.0962238609790802
1200 0.0978318601846695
1220 0.0996112823486328
1240 0.101423874497414
1260 0.103104338049889
1280 0.104620359838009
1300 0.106012284755707
1320 0.107281923294067
1340 0.108633667230606
1360 0.110000908374786
1380 0.111493661999702
1400 0.113005131483078
1420 0.114599525928497
1440 0.116065889596939
1460 0.117480181157589
1480 0.118752330541611
1500 0.119964703917503
1520 0.121093437075615
1540 0.122234247624874
1560 0.123457074165344
1580 0.124654874205589
1600 0.125847667455673
1620 0.126990675926208
1640 0.128143951296806
1660 0.129189699888229
1680 0.130227208137512
1700 0.131150335073471
1720 0.132109016180038
1740 0.133057996630669
1760 0.133972689509392
1780 0.134979546070099
1800 0.135939627885818
1820 0.137014359235764
1840 0.138141706585884
1860 0.139159247279167
1880 0.140270441770554
1900 0.141322076320648
1920 0.142257243394852
1940 0.143254056572914
1960 0.144155263900757
1980 0.144944697618484
2000 0.145886570215225
2020 0.146861553192139
2040 0.14788793027401
2060 0.149084240198135
2080 0.150266319513321
2100 0.151428923010826
2120 0.152640014886856
2140 0.15384829044342
2160 0.155017271637917
2180 0.156187757849693
2200 0.157341659069061
2220 0.158453345298767
2240 0.159551307559013
2260 0.160668566823006
2280 0.161829560995102
2300 0.16300755739212
2320 0.164137840270996
2340 0.165277689695358
2360 0.166451379656792
2380 0.167552977800369
2400 0.168535828590393
2420 0.169487357139587
2440 0.170421600341797
2460 0.171289443969727
2480 0.172094196081161
2500 0.172876998782158
2520 0.173627197742462
2540 0.174336835741997
2560 0.17502461373806
2580 0.175691530108452
2600 0.176343485713005
2620 0.176955580711365
2640 0.177586764097214
2660 0.178266450762749
2680 0.178917944431305
2700 0.17950439453125
2720 0.180041655898094
2740 0.180602431297302
2760 0.181182980537415
2780 0.181729197502136
2800 0.182235866785049
2820 0.182753682136536
2840 0.183320283889771
2860 0.18388769030571
2880 0.184383377432823
2900 0.184820115566254
2920 0.185236185789108
2940 0.185658067464828
2960 0.18607372045517
2980 0.186444208025932
};
\addlegendentry{nDGGNN }
\addplot [semithick, red, mark=*, mark size=2.5, mark repeat=20, mark options={solid,fill=white}]
table {%
0 0
20 0.00737858098000288
40 0.0124447625130415
60 0.0125109236687422
80 0.00973169133067131
100 0.00953830406069756
120 0.00986992474645376
140 0.010861910879612
160 0.0103404624387622
180 0.0115247992798686
200 0.0116180777549744
220 0.0124141899868846
240 0.0129668302834034
260 0.0133319785818458
280 0.0140674989670515
300 0.0145957451313734
320 0.0150305880233645
340 0.0153874140232801
360 0.0160251744091511
380 0.0166112799197435
400 0.0168754234910011
420 0.0175752323120832
440 0.0184061955660582
460 0.0189797170460224
480 0.0194562301039696
500 0.020002081990242
520 0.0204297285526991
540 0.0205662176012993
560 0.0204802490770817
580 0.0202650930732489
600 0.0200392957776785
620 0.0197138823568821
640 0.0192395858466625
660 0.0186593737453222
680 0.0180492643266916
700 0.0174408107995987
720 0.0168164204806089
740 0.0161308329552412
760 0.0154475327581167
780 0.0149169247597456
800 0.0145251378417015
820 0.0141579983755946
840 0.013783723115921
860 0.0133917517960072
880 0.0130558777600527
900 0.0128808422014117
920 0.0128067340701818
940 0.0128251239657402
960 0.0128536317497492
980 0.0128490058705211
1000 0.0128005174919963
1020 0.0127545185387135
1040 0.0128328008577228
1060 0.0129512054845691
1080 0.0131081137806177
1100 0.0132414288818836
1120 0.0133097376674414
1140 0.0133315231651068
1160 0.0133447851985693
1180 0.0134024266153574
1200 0.0135595574975014
1220 0.0137339346110821
1240 0.0138403698801994
1260 0.0139567907899618
1280 0.0139892315492034
1300 0.0140376780182123
1320 0.0140135176479816
1340 0.0139892976731062
1360 0.0139882285147905
1380 0.0139937549829483
1400 0.0140830166637897
1420 0.0141073688864708
1440 0.0140713658183813
1460 0.0140258874744177
1480 0.0140027478337288
1500 0.0139457155019045
1520 0.0138934012502432
1540 0.0138104427605867
1560 0.0137507729232311
1580 0.0137010663747787
1600 0.0136653129011393
1620 0.0135760884732008
1640 0.0134788518771529
1660 0.0132744526490569
1680 0.0131904948502779
1700 0.0130450678989291
1720 0.0129961250349879
1740 0.0129241263493896
1760 0.0128457322716713
1780 0.0128279682248831
1800 0.0127173475921154
1820 0.0126946121454239
1840 0.0126581415534019
1860 0.012587851844728
1880 0.0125665720552206
1900 0.0124930161982775
1920 0.0124292923137546
1940 0.0124263493344188
1960 0.0123515455052257
1980 0.0123659987002611
2000 0.0124386623501778
2020 0.0124428225681186
2040 0.0125410724431276
2060 0.0125564187765121
2080 0.01252163015306
2100 0.0126018999144435
2120 0.0126329679042101
2140 0.0126243708655238
2160 0.0127614652737975
2180 0.0128892688080668
2200 0.0129073224961758
2220 0.0130045432597399
2240 0.0131556643173099
2260 0.0132403131574392
2280 0.0132999522611499
2300 0.0134071838110685
2320 0.0134926624596119
2340 0.013531468808651
2360 0.0135524570941925
2380 0.0136177940294147
2400 0.0136523321270943
2420 0.0136385429650545
2440 0.0136603964492679
2460 0.0137565499171615
2480 0.0137788914144039
2500 0.0138089936226606
2520 0.0139311952516437
2540 0.0140795288607478
2560 0.0141754280775785
2580 0.0142637519165874
2600 0.0143985021859407
2620 0.0145225552842021
2640 0.0145530700683594
2660 0.0145503263920546
2680 0.0145641518756747
2700 0.0145988911390305
2720 0.0145665500313044
2740 0.0145471021533012
2760 0.014593968167901
2780 0.0146887553855777
2800 0.0147590413689613
2820 0.0148269087076187
2840 0.0149083007127047
2860 0.0150242699310184
2880 0.0151345087215304
2900 0.0151842664927244
2920 0.0152342896908522
2940 0.0153142306953669
2960 0.0154129955917597
2980 0.0154951391741633
};
\addlegendentry{mcDGGNN ($11\%$) }
\end{axis}

\end{tikzpicture}


==> Figs/2D_cross_solving/Error_cross_solving.tex <==
\begin{tabular}{l||c c c c c}
\toprule
{} & Forward & Scramjet & Airfoil & Euler-config6 & Double Mach Reflection \\
\midrule
Forward - nDGGNN        &  0.0349 &   0.0819 &  0.0105 &        0.2336 &      0.1336 \\
Forward - mcDGGNN       &  0.0131 &   0.0848 &  0.0033 &        0.0993 &      0.0403 \\
Scramjet - nDGGNN       &  0.0140 &   0.0812 &  0.0055 &        0.0866 &      0.0947 \\
Scramjet - mcDGGNN      &  0.0154 &   0.0109 &  0.0037 &        0.0936 &      0.0546 \\
Airfoil - nDGGNN        &  0.0767 &   0.1530 &  0.0031 &        0.6193 &      0.2888 \\
Airfoil - mcDGGNN       &  0.0557 &   0.1124 &  0.0017 &        0.3048 &      0.0577 \\
Euler-config6 - nDGGNN  &  0.0629 &   0.0618 &  0.0083 &        0.1623 &      0.1691 \\
Euler-config6 - mcDGGNN &  0.0603 &   0.0993 &  0.0018 &        0.0229 &      0.0522 \\
Double Mach Reflection - nDGGNN    &  0.1180 &   0.0855 &  0.0137 &        0.1528 &      0.0168 \\
Double Mach Reflection - mcDGGNN   &  0.1400 &   0.0663 &  0.0121 &        0.1499 &      0.0171 \\
\bottomrule
\end{tabular}


==> Figs/Architecture_DGblock.tex <==
\begin{tikzpicture}[
    node distance=\layersep,
    edge/.style={-stealth,shorten >=1pt, draw=black!50,thin},
    neuron/.style={circle,fill=black!25,minimum size=10pt,inner sep=0pt},
    operator/.style={rectangle,fill=green!,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, inner sep=0pt, rounded corners},
    input neuron/.style={neuron, fill=green!50,minimum size=12pt},
    output neuron/.style={neuron, fill=green!50,minimum size=12pt},
    hidden neuron/.style={neuron, fill=blue!50},
    Forward map/.style={operator, fill=red!50},
    annot/.style={text width=4em, text centered},
    every node/.style={scale=1.0},
    node1/.style={scale=2.0},
    cross/.style={path picture={ \draw[black, shorten <=2pt, shorten >=2pt, line width=1pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw[black, shorten <=2pt, shorten >=2pt, line width=1pt] (path picture bounding box.west) -- (path picture bounding box.east);}}
]

\draw[draw=blue, thick, fill=blue!5, rounded corners] (-.5*\layersep, -9.4*\nodeinlayersep) rectangle (6.3*\layersep, -0.2*\nodeinlayersep);
\draw[draw=black!50,thick, dashed] (-2.2*\layersep, -3.9*\nodeinlayersep) -- (6.5*\layersep, -3.9*\nodeinlayersep); 
\node [align=left](Node Level) at (-1.7*\layersep, -3.2*\nodeinlayersep) {Node Level };

\node [align=left](Edge Level) at (-1.7*\layersep, -4.7*\nodeinlayersep) {Edge Level};

\node[rectangle, draw = black,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (u_in) at (-1.1*\layersep, -2*\nodeinlayersep) {$\ub^{{k}}$};

\node[rectangle, draw = black,fill=white!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fu) at (2.*\layersep, -2*\nodeinlayersep) {$\fb^{k}$};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (volintegration) at (4.*\layersep, -2*\nodeinlayersep) {$\LRp{M^k}^{-1} \int_{\Omega^k} \NNvol \LRp{\fb^k} \pp{\phi\LRp{\xb}}{\xb} d\xb$};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fluxintegration) at (4.*\layersep, -7*\nodeinlayersep) {$-\LRp{M^k}^{-1} \int_{\partial\Omega^k}  \nb \cdot \fb^* \phi\LRp{\xb} d\xb$};


\node[rectangle, draw = black,fill=white!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (volintegration) at (4.5*\layersep, -2*\nodeinlayersep) {$\sum_{i}^d V_i^k \LRs{\boldsymbol{\eta}^k \NNvol \LRp{\overline{\fb}^k}}_i $};

\node[rectangle, draw = black,fill=white!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fluxintegration) at (4.7*\layersep, -8.4*\nodeinlayersep) {$ - \sum_{e} E^{k,e} \LRp{\nb \cdot \fb^*}$};

\node[rectangle, draw = black,fill=white!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners, align=center] (flux_ML) at (1.3*\layersep, -8.4*\nodeinlayersep) 
{$\LRp{\nb \cdot \fb^*}  = \boldsymbol{\psi}^e \NNflux \LRp{\overline{\nb \odot \dLRc{\fb^e}}, \overline{\dLRs{\ub^e}}}$};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners, align=center] (u_in) at (-1.2*\layersep, -2*\nodeinlayersep) {Line 1 \\ Line 2};

\draw[edge,thin] (u_in) -- (fu);
\draw[edge,thin] (fu) -- (volintegration);
\draw[edge,thin] (fu) -- (2.*\layersep, -7.7*\nodeinlayersep);
\draw[edge,thin] (0.6*\layersep, -2.*\nodeinlayersep) -- (0.6*\layersep, -7.7*\nodeinlayersep);

\draw[edge,thin] (flux_ML) -- (fluxintegration);


\node[rectangle, draw = black,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (0.6*\layersep, -4.8*\nodeinlayersep) {$\dLRs{\ub^e}$};

\node[rectangle, draw = black,fill=white!100,minimum height= \nodeinlayersep, minimum width= 1.8 * \layersep, rounded corners] at (1.25*\layersep, -6.45*\nodeinlayersep) {normalization};

\node[rectangle, draw = black,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (2.*\layersep, -4.8*\nodeinlayersep) {$\dLRc{\fb^e}$};

\node [draw,circle,cross,minimum width=.02*\layersep,line width=.3pt](cross_1) at (6.*\layersep, -2*\nodeinlayersep){};

\node[rectangle, draw = black, rotate = 90,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (2.9*\layersep, -2*\nodeinlayersep) {normalization};

\draw[edge,thin] (fluxintegration) -- (6.*\layersep, -8.4*\nodeinlayersep) -- (cross_1);
\draw[edge,thin] (volintegration) -- (cross_1);
\draw[edge,thin] (cross_1) -- (6.6*\layersep, -2*\nodeinlayersep);


\end{tikzpicture}







% \begin{figure}[htb!]
% \centering
% \def\layersep{2.cm}
% \def\nodeinlayersep{0.8cm}
% \usetikzlibrary{calc}
% \begin{tikzpicture}[
%     node distance=\layersep,
%     edge/.style={-stealth,shorten >=1pt, draw=black!50,thin},
%     neuron/.style={circle,fill=black!25,minimum size=10pt,inner sep=0pt},
%     operator/.style={rectangle,fill=green!,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, inner sep=0pt, rounded corners},
%     input neuron/.style={neuron, fill=green!50,minimum size=12pt},
%     output neuron/.style={neuron, fill=green!50,minimum size=12pt},
%     hidden neuron/.style={neuron, fill=blue!50},
%     Forward map/.style={operator, fill=red!50},
%     annot/.style={text width=4em, text centered},
%     every node/.style={scale=1.0},
%     node1/.style={scale=2.0},
%     cross/.style={path picture={ \draw[black, shorten <=2pt, shorten >=2pt, line width=1pt] (path picture bounding box.south) -- (path picture bounding box.north); \draw[black, shorten <=2pt, shorten >=2pt, line width=1pt] (path picture bounding box.west) -- (path picture bounding box.east);}}
% ]

% \node (Node) at (-2.2*\layersep, -2*\nodeinlayersep) {Node};

% \node (Edge) at (-2.2*\layersep, -7*\nodeinlayersep) {Edge};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (u_in) at (-1.2*\layersep, -2*\nodeinlayersep) {$\ub^{{k}}$};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fu) at (2.*\layersep, -2*\nodeinlayersep) {$\fb^{k}$};

% % \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (volintegration) at (4.*\layersep, -2*\nodeinlayersep) {$\LRp{M^k}^{-1} \int_{\Omega^k} \NNvol \LRp{\fb^k} \pp{\phi\LRp{\xb}}{\xb} d\xb$};

% % \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fluxintegration) at (4.*\layersep, -7*\nodeinlayersep) {$-\LRp{M^k}^{-1} \int_{\partial\Omega^k}  \nb \cdot \fb^* \phi\LRp{\xb} d\xb$};


% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (volintegration) at (4.5*\layersep, -2*\nodeinlayersep) {$\sum_{i}^d V_i^k \LRs{\boldsymbol{\eta}^k \NNvol \LRp{\overline{\fb}^k}}_i $};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (fluxintegration) at (4.5*\layersep, -7*\nodeinlayersep) {$-E^k \LRp{\nb \cdot \fb^*}$};

% \node[rectangle,fill=yellow!50,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] (flux_ML) at (1.3*\layersep, -7*\nodeinlayersep) {$\nb \cdot \fb^* = \boldsymbol{\psi} \NNflux \LRp{\overline{\nb \odot \dLRc{\fb}}, \overline{\dLRs{\ub}}}$};

% \draw[edge,thin] (u_in) -- (fu);
% \draw[edge,thin] (fu) -- (volintegration);
% \draw[edge,thin] (fu) -- (2.*\layersep, -6.5*\nodeinlayersep);
% \draw[edge,thin] (0.6*\layersep, -2.*\nodeinlayersep) -- (0.6*\layersep, -6.5*\nodeinlayersep);

% \draw[edge,thin] (flux_ML) -- (fluxintegration);


% \node[rectangle,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (0.5*\layersep, -3.5*\nodeinlayersep) {$\dLRs{\ub}^{\LRp{k, \mc{N}\LRp{k}}}$};

% \node[rectangle, draw = black,fill=white!100,minimum height= \nodeinlayersep, minimum width= 1.8 * \layersep, rounded corners] at (1.25*\layersep, -5.25*\nodeinlayersep) {normalization};

% \node[rectangle,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (2.*\layersep, -3.5*\nodeinlayersep) {$\dLRc{\fb}^{\LRp{k, \mc{N}\LRp{k}}}$};

% \node [draw,circle,cross,minimum width=.02*\layersep,line width=.3pt](cross_1) at (6.*\layersep, -2*\nodeinlayersep){};

% \node[rectangle, draw = black, rotate = 90,fill=white!100,minimum height= \nodeinlayersep, minimum width= 0.8 * \layersep, rounded corners] at (2.9*\layersep, -2*\nodeinlayersep) {normalization};

% \draw[edge,thin] (fluxintegration) -- (6.*\layersep, -7*\nodeinlayersep) -- (cross_1);
% \draw[edge,thin] (volintegration) -- (cross_1);
% \draw[edge,thin] (cross_1) -- (6.6*\layersep, -2*\nodeinlayersep);

% \draw[draw=blue, thick] (-.5*\layersep, -7.9*\nodeinlayersep) rectangle (6.3*\layersep, -0.2*\nodeinlayersep);

% \end{tikzpicture}
% \caption{Description of $\DGGNN$  architecture block for an element $k$. At the node level, the element nodal values $\ub^k$ serve as node attributes in the graph neural network framework. The whole element flux vector ${\fb}^k$ is evaluated algebraically from $\ub^k$ and then is normalized to from $\overline{\fb}^k$ as in \cref{eq:normalized_vol}. The network $\NNvol$ modifies the normalized flux to learn the corrections. The output is denormalized by factor $\boldsymbol{\eta}^k$. Finally, we apply the collocation-type integration rule to compute the volume term. At the edge level, $\NNflux$ represents the graph neural network edges. It computes the numerical fluxes at the shared edge points of the element $k$ and its adjacent elements $\mc{N}\LRp{k}$. The input for $\NNflux$ comprises the normalized average flux terms $\overline{\nb \cdot \dLRc{\fb}}^{\left(k, \mathcal{N}\left(k\right)\right)}$ and normalized state jump $\overline{\dLRs{\ub}}^{\left(k, \mathcal{N}\left(k\right)\right)}$ computed as in \cref{eq:normalized_flux}. The output of the numerical flux network is denormalized by factor $\boldsymbol{\psi}$ to evaluate the numerical flux at the corresponding edge point. Subsequently, the approximated numerical fluxes undergo a collocation-type integration rule for evaluating the flux term. The flux and volume terms are added up to return the tangent slope on for the $k-$element.}
% \figlab{NN_block_architecture}
% \end{figure}




==> Figs/Isentropic_vortex/rho_convergence_rate.tex <==
\begin{tabular}{l||c c c | c || c c c | c}
\toprule
{} &         h &       h/2 &       h/4 &      Rate &         h &       h/2 &       h/4 &      Rate \\
\midrule
N = 1 &  6.32e-02 &  2.51e-02 &  7.51e-03 &  1.55e+00 &  1.09e-01 &  4.62e-02 &  1.11e-02 &  1.66e+00 \\
N = 2 &  1.95e-02 &  4.43e-03 &  8.58e-04 &  2.25e+00 &  4.30e-02 &  8.55e-03 &  1.48e-03 &  2.43e+00 \\
N = 3 &  6.71e-03 &  7.58e-04 &  8.20e-05 &  3.18e+00 &  1.39e-02 &  1.45e-03 &  1.12e-04 &  3.48e+00 \\
N = 4 &  2.58e-03 &  1.46e-04 &  7.65e-06 &  4.20e+00 &  4.93e-03 &  2.06e-04 &  9.61e-06 &  4.50e+00 \\
N = 1 &  6.32e-02 &  2.49e-02 &  7.22e-03 &  1.57e+00 &  1.11e-01 &  4.72e-02 &  1.12e-02 &  1.66e+00 \\
N = 2 &  1.96e-02 &  4.35e-03 &  9.29e-04 &  2.20e+00 &  4.39e-02 &  8.33e-03 &  1.48e-03 &  2.45e+00 \\
N = 3 &  6.77e-03 &  7.53e-04 &  8.20e-05 &  3.18e+00 &  1.35e-02 &  1.45e-03 &  1.12e-04 &  3.46e+00 \\
N = 4 &  2.77e-03 &  1.46e-04 &  8.65e-06 &  4.17e+00 &  4.96e-03 &  2.07e-04 &  1.03e-05 &  4.45e+00 \\
\bottomrule
\end{tabular}


==> Figs/Isentropic_vortex/rho_convergence_rate_N3h16.tex <==
\begin{tabular}{l||c c c | c || c c c | c}
\toprule
{} &         h &       h/2 &       h/4 &      Rate &         h &       h/2 &       h/4 &      Rate \\
\midrule
N = 1 &  6.32e-02 &  2.51e-02 &  7.51e-03 &  1.55e+00 &  1.09e-01 &  4.62e-02 &  1.11e-02 &  1.66e+00 \\
N = 2 &  1.95e-02 &  4.43e-03 &  8.58e-04 &  2.25e+00 &  4.30e-02 &  8.55e-03 &  1.48e-03 &  2.43e+00 \\
N = 3 &  6.71e-03 &  7.58e-04 &  8.20e-05 &  3.18e+00 &  1.39e-02 &  1.45e-03 &  1.12e-04 &  3.48e+00 \\
N = 4 &  2.58e-03 &  1.46e-04 &  7.65e-06 &  4.20e+00 &  4.93e-03 &  2.06e-04 &  9.61e-06 &  4.50e+00 \\
N = 1 &  7.64e-02 &  3.30e-02 &  9.36e-03 &  1.53e+00 &  1.32e-01 &  5.98e-02 &  1.41e-02 &  1.62e+00 \\
N = 2 &  2.36e-02 &  4.61e-03 &  9.29e-04 &  2.33e+00 &  5.07e-02 &  8.63e-03 &  1.48e-03 &  2.55e+00 \\
N = 3 &  7.50e-03 &  8.86e-04 &  3.54e-04 &  2.20e+00 &  1.39e-02 &  1.49e-03 &  3.19e-04 &  2.72e+00 \\
N = 4 &  3.03e-03 &  2.62e-04 &  4.23e-04 &  1.42e+00 &  4.99e-03 &  2.76e-04 &  3.67e-04 &  1.88e+00 \\
\bottomrule
\end{tabular}


==> Figs/Isentropic_vortex/rho_convergence_rate_N3h4_forall.tex <==
\begin{tabular}{l||c c c | c || c c c | c}
\toprule
{} &         h &       h/2 &       h/4 &       Rate &         h &       h/2 &       h/4 &       Rate \\
\midrule
N = 1 &  6.32e-02 &  2.51e-02 &  7.51e-03 &   1.55e+00 &  1.09e-01 &  4.62e-02 &  1.11e-02 &   1.66e+00 \\
N = 2 &  1.95e-02 &  4.43e-03 &  8.58e-04 &   2.25e+00 &  4.30e-02 &  8.55e-03 &  1.48e-03 &   2.43e+00 \\
N = 3 &  6.71e-03 &  7.58e-04 &  8.20e-05 &   3.18e+00 &  1.39e-02 &  1.45e-03 &  1.12e-04 &   3.48e+00 \\
N = 4 &  2.58e-03 &  1.46e-04 &  7.65e-06 &   4.20e+00 &  4.93e-03 &  2.06e-04 &  9.61e-06 &   4.50e+00 \\
N = 1 &  6.38e-02 &  2.49e-02 &  7.60e-03 &   1.54e+00 &  1.11e-01 &  4.70e-02 &  1.11e-02 &   1.67e+00 \\
N = 2 &  1.96e-02 &  5.05e-03 &  5.03e-03 &   9.77e-01 &  4.39e-02 &  8.65e-03 &  5.18e-03 &   1.54e+00 \\
N = 3 &  6.88e-03 &  3.31e-03 &  6.91e-03 &  -7.21e-03 &  1.36e-02 &  3.39e-03 &  7.04e-03 &   4.69e-01 \\
N = 4 &  3.22e-03 &  4.07e-03 &  8.46e-03 &  -6.97e-01 &  5.15e-03 &  4.23e-03 &  9.09e-03 &  -4.15e-01 \\
\bottomrule
\end{tabular}


==> Figs/Isentropic_vortex/rho_convergence_rate_N3h8_forall.tex <==
\begin{tabular}{l||c c c | c || c c c | c}
\toprule
{} &         h &       h/2 &       h/4 &      Rate &         h &       h/2 &       h/4 &      Rate \\
\midrule
N = 1 &  6.32e-02 &  2.51e-02 &  7.51e-03 &  1.55e+00 &  1.09e-01 &  4.62e-02 &  1.11e-02 &  1.66e+00 \\
N = 2 &  1.95e-02 &  4.43e-03 &  8.58e-04 &  2.25e+00 &  4.30e-02 &  8.55e-03 &  1.48e-03 &  2.43e+00 \\
N = 3 &  6.71e-03 &  7.58e-04 &  8.20e-05 &  3.18e+00 &  1.39e-02 &  1.45e-03 &  1.12e-04 &  3.48e+00 \\
N = 4 &  2.58e-03 &  1.46e-04 &  7.65e-06 &  4.20e+00 &  4.93e-03 &  2.06e-04 &  9.61e-06 &  4.50e+00 \\
N = 1 &  6.54e-02 &  2.57e-02 &  7.19e-03 &  1.60e+00 &  1.14e-01 &  4.83e-02 &  1.12e-02 &  1.68e+00 \\
N = 2 &  2.00e-02 &  4.35e-03 &  9.74e-04 &  2.18e+00 &  4.45e-02 &  8.33e-03 &  1.57e-03 &  2.42e+00 \\
N = 3 &  6.73e-03 &  8.40e-04 &  6.30e-04 &  1.71e+00 &  1.35e-02 &  1.47e-03 &  8.11e-04 &  2.03e+00 \\
N = 4 &  2.62e-03 &  4.55e-04 &  7.87e-04 &  8.69e-01 &  4.83e-03 &  6.30e-04 &  1.00e-03 &  1.13e+00 \\
\bottomrule
\end{tabular}


==> Figs/Isentropic_vortex/style.tex <==
\begin{tabular}{l|c c c | c | c c c | c|}
    \toprule
    \multicolumn{1}{l|}{} & \multicolumn{4}{c|}{$\rho$}  & \multicolumn{4}{c|}{$\rho u$}  \\
    \midrule
    {} &         h &       h/2 &       h/4 &      Rate &         h &       h/2 &       h/4 &      Rate \\
    \midrule
    \midrule
    \multicolumn{1}{l}{} & \multicolumn{8}{c}{DG}  \\
    \midrule
    N = 1 &  1.09e-01 &  3.03e-02 &  8.29e-03 &  1.87e+00 &  1.80e-01 &  4.92e-02 &  1.20e-02 &  2.03e+00 \\
    N = 2 &  3.37e-02 &  8.02e-03 &  1.72e-03 &  2.22e+00 &  6.24e-02 &  1.20e-02 &  2.48e-03 &  2.27e+00 \\
    N = 3 &  1.80e-02 &  1.99e-03 &  1.38e-04 &  3.86e+00 &  2.44e-02 &  2.23e-03 &  1.81e-04 &  3.62e+00 \\
    \midrule
    \midrule
    \multicolumn{1}{l}{} & \multicolumn{8}{c}{DGGNN 0.2\% noise}  \\
    \midrule
    N = 1 &  1.08e-01 &  3.09e-02 &  8.67e-03 &  1.83e+00 &  1.81e-01 &  5.00e-02 &  1.23e-02 &  2.03e+00 \\
    N = 2 &  3.34e-02 &  8.04e-03 &  2.00e-03 &  2.01e+00 &  6.23e-02 &  1.20e-02 &  2.57e-03 &  2.22e+00 \\
    N = 3 &  1.80e-02 &  2.04e-03 &  1.67e-04 &  3.62e+00 &  2.41e-02 &  2.25e-03 &  1.94e-04 &  3.54e+00 \\
\bottomrule
\end{tabular}


==> Figs/data_noise/image_dual_mesh.tex <==



\tikzset{every picture/.style={line width=0.75pt}} %set default line width to 0.75pt        

\begin{tikzpicture}[x=0.75pt,y=0.75pt,yscale=-1,xscale=1]
%uncomment if require: \path (0,915); %set diagram left start at 0, and has height of 915

%Shape: Polygon [id:dp007081578378051123] 
\draw   (449,245.99) -- (412.49,355.59) -- (316.91,423.32) -- (198.76,423.32) -- (103.18,355.59) -- (66.67,245.99) -- (103.18,136.39) -- (198.76,68.66) -- (316.91,68.66) -- (412.49,136.39) -- cycle ;
%Straight Lines [id:da2620246486921629] 
\draw    (198.76,68.66) -- (316.91,423.32) ;
%Straight Lines [id:da6533650368561275] 
\draw    (103.18,138.39) -- (198.76,425.32) ;
%Straight Lines [id:da4825040826538276] 
\draw    (316.91,70.66) -- (412.49,357.59) ;
%Straight Lines [id:da4564277082660322] 
\draw    (66.67,247.99) -- (412.49,138.39) ;
%Straight Lines [id:da6973006202056349] 
\draw    (103.18,357.59) -- (449,247.99) ;
%Straight Lines [id:da664226146898625] 
\draw    (103.18,138.39) -- (316.91,70.66) ;
%Straight Lines [id:da36316261801535243] 
\draw    (198.76,423.32) -- (412.49,355.59) ;
%Straight Lines [id:da7050387244593386] 
\draw    (239.58,193.19) -- (316.91,70.66) ;
%Straight Lines [id:da479220951561121] 
\draw    (276.09,302.79) -- (345.88,158.92) ;
%Straight Lines [id:da21219791707190794] 
\draw    (305.63,391.46) -- (383.64,267.29) ;
%Straight Lines [id:da9553292005533656] 
\draw    (383.64,267.29) -- (412.49,138.39) ;
%Straight Lines [id:da5039763752468287] 
\draw    (239.58,193.19) -- (103.18,138.39) ;
%Straight Lines [id:da7886003325403008] 
\draw    (276.09,302.79) -- (132.39,226.92) ;
%Straight Lines [id:da4314685157368061] 
\draw    (305.63,391.46) -- (169.42,336) ;
%Straight Lines [id:da47516117108181266] 
\draw    (169.42,336) -- (66.67,247.99) ;
%Shape: Polygon [id:dp5392847327151786] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (293.09,219.34) -- (289.39,225.6) -- (281.98,225.6) -- (278.28,219.34) -- (281.98,213.08) -- (289.39,213.08) -- cycle ;
%Shape: Polygon [id:dp5878240264387642] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (347.55,248.38) -- (343.85,254.64) -- (336.44,254.64) -- (332.74,248.38) -- (336.44,242.12) -- (343.85,242.12) -- cycle ;
%Shape: Polygon [id:dp08328994398266376] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (386.77,182.51) -- (383.06,188.76) -- (375.66,188.76) -- (371.95,182.51) -- (375.66,176.25) -- (383.06,176.25) -- cycle ;
%Shape: Polygon [id:dp04397100424252942] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (423.08,222.88) -- (419.37,229.14) -- (411.96,229.14) -- (408.26,222.88) -- (411.96,216.62) -- (419.37,216.62) -- cycle ;
%Shape: Polygon [id:dp050351256296331526] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (422.35,290.17) -- (418.65,296.43) -- (411.24,296.43) -- (407.54,290.17) -- (411.24,283.91) -- (418.65,283.91) -- cycle ;
%Shape: Polygon [id:dp38424262674983845] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (377.33,336.92) -- (373.62,343.17) -- (366.22,343.17) -- (362.51,336.92) -- (366.22,330.66) -- (373.62,330.66) -- cycle ;
%Shape: Polygon [id:dp43392918844007533] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (345.37,395.71) -- (341.67,401.96) -- (334.26,401.96) -- (330.56,395.71) -- (334.26,389.45) -- (341.67,389.45) -- cycle ;
%Shape: Polygon [id:dp6281234561793814] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (286.55,411.41) -- (282.85,417.67) -- (275.44,417.67) -- (271.74,411.41) -- (275.44,405.16) -- (282.85,405.16) -- cycle ;
%Shape: Polygon [id:dp005386780081995113] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (229.19,385.08) -- (225.48,391.34) -- (218.08,391.34) -- (214.37,385.08) -- (218.08,378.82) -- (225.48,378.82) -- cycle ;
%Shape: Polygon [id:dp11887155090541635] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (263.32,344) -- (259.61,350.26) -- (252.21,350.26) -- (248.5,344) -- (252.21,337.74) -- (259.61,337.74) -- cycle ;
%Shape: Polygon [id:dp29713670540153414] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (323.59,322.04) -- (319.89,328.3) -- (312.48,328.3) -- (308.77,322.04) -- (312.48,315.79) -- (319.89,315.79) -- cycle ;
%Shape: Polygon [id:dp2267220997820094] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (225.55,235.63) -- (221.85,241.89) -- (214.44,241.89) -- (210.74,235.63) -- (214.44,229.37) -- (221.85,229.37) -- cycle ;
%Shape: Polygon [id:dp362363213422525] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (201.59,293.71) -- (197.89,299.97) -- (190.48,299.97) -- (186.78,293.71) -- (190.48,287.45) -- (197.89,287.45) -- cycle ;
%Shape: Polygon [id:dp6057578619364576] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (126.07,264.67) -- (122.36,270.93) -- (114.96,270.93) -- (111.25,264.67) -- (114.96,258.41) -- (122.36,258.41) -- cycle ;
%Shape: Polygon [id:dp18583976945172465] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (122.44,316.38) -- (118.73,322.63) -- (111.33,322.63) -- (107.62,316.38) -- (111.33,310.12) -- (118.73,310.12) -- cycle ;
%Shape: Polygon [id:dp7375326079197126] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (162.38,367.37) -- (158.67,373.63) -- (151.27,373.63) -- (147.56,367.37) -- (151.27,361.12) -- (158.67,361.12) -- cycle ;
%Shape: Polygon [id:dp12333599982046439] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (110.09,208.71) -- (106.39,214.97) -- (98.98,214.97) -- (95.28,208.71) -- (98.98,202.46) -- (106.39,202.46) -- cycle ;
%Shape: Polygon [id:dp9244450250967278] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (161.65,188.88) -- (157.95,195.14) -- (150.54,195.14) -- (146.84,188.88) -- (150.54,182.63) -- (157.95,182.63) -- cycle ;
%Shape: Polygon [id:dp20525802174825714] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (258.23,123.01) -- (254.53,129.27) -- (247.12,129.27) -- (243.42,123.01) -- (247.12,116.75) -- (254.53,116.75) -- cycle ;
%Shape: Polygon [id:dp9189844998463166] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (313.42,142.84) -- (309.72,149.1) -- (302.31,149.1) -- (298.61,142.84) -- (302.31,136.59) -- (309.72,136.59) -- cycle ;
%Shape: Polygon [id:dp33570336277029433] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (367.16,125.84) -- (363.46,132.1) -- (356.05,132.1) -- (352.35,125.84) -- (356.05,119.59) -- (363.46,119.59) -- cycle ;
%Shape: Polygon [id:dp11860105399888088] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (236.45,84.76) -- (232.74,91.02) -- (225.34,91.02) -- (221.63,84.76) -- (225.34,78.51) -- (232.74,78.51) -- cycle ;
%Shape: Polygon [id:dp042453193801588185] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (189.97,98.93) -- (186.27,105.19) -- (178.86,105.19) -- (175.16,98.93) -- (178.86,92.67) -- (186.27,92.67) -- cycle ;
%Shape: Polygon [id:dp2070513922599282] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (202.32,140.72) -- (198.61,146.97) -- (191.21,146.97) -- (187.5,140.72) -- (191.21,134.46) -- (198.61,134.46) -- cycle ;
%Straight Lines [id:da40022051069375375] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (182.56,98.93) -- (194.91,140.72) ;
%Straight Lines [id:da9047233344947561] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (229.04,84.76) -- (250.83,123.01) ;
%Straight Lines [id:da03775750802523237] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (250.83,123.01) -- (194.91,140.72) ;
%Straight Lines [id:da020006028965888545] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (306.02,142.84) -- (285.68,219.34) ;
%Straight Lines [id:da06902875672774655] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (250.83,123.01) -- (306.02,142.84) ;
%Straight Lines [id:da7255084159213492] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (306.02,142.84) -- (359.75,125.84) ;
%Straight Lines [id:da3289454941504599] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (379.36,182.51) -- (359.75,125.84) ;
%Straight Lines [id:da38559495643865294] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (415.67,222.88) -- (379.36,182.51) ;
%Straight Lines [id:da6608382166241697] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (379.36,182.51) -- (340.15,248.38) ;
%Straight Lines [id:da05975512309297626] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (340.15,248.38) -- (285.68,219.34) ;
%Straight Lines [id:da8642369500990319] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (316.18,322.04) -- (340.15,248.38) ;
%Straight Lines [id:da6931764413438575] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (369.92,336.92) -- (316.18,322.04) ;
%Straight Lines [id:da39984560106402744] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (414.94,290.17) -- (415.67,222.88) ;
%Straight Lines [id:da9155127935973346] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (369.92,336.92) -- (414.94,290.17) ;
%Straight Lines [id:da7675379304986945] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (337.97,395.71) -- (369.92,336.92) ;
%Straight Lines [id:da4993464090191002] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (255.91,344) -- (316.18,322.04) ;
%Straight Lines [id:da8791511939690824] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (221.78,385.08) -- (255.91,344) ;
%Straight Lines [id:da70597235526877] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (221.78,385.08) -- (279.15,413.41) ;
%Straight Lines [id:da5068964228114465] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (279.15,413.41) -- (337.97,395.71) ;
%Straight Lines [id:da2633732896361791] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (218.15,235.63) -- (285.68,219.34) ;
%Straight Lines [id:da8209555276919605] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (194.18,293.71) -- (218.15,235.63) ;
%Straight Lines [id:da29602013290904194] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (255.91,344) -- (194.18,293.71) ;
%Straight Lines [id:da4744428029845402] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (221.78,385.08) -- (154.97,367.37) ;
%Straight Lines [id:da5763497245239375] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (154.97,367.37) -- (115.03,316.38) ;
%Straight Lines [id:da4239203618622598] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (115.03,316.38) -- (118.66,264.67) ;
%Straight Lines [id:da425663482763172] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (194.18,293.71) -- (118.66,264.67) ;
%Straight Lines [id:da4125717621266405] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (118.66,264.67) -- (102.69,208.71) ;
%Straight Lines [id:da5185042982728121] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (102.69,208.71) -- (154.24,188.88) ;
%Straight Lines [id:da930531301598404] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (154.24,188.88) -- (194.91,140.72) ;
%Straight Lines [id:da2004567417496932] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (154.24,188.88) -- (218.15,235.63) ;
%Straight Lines [id:da4108254161330174] 
\draw [color={rgb, 255:red, 245; green, 166; blue, 35 }  ,draw opacity=1 ]   (182.56,98.93) -- (229.04,84.76) ;
%Shape: Regular Polygon [id:dp7787625451480442] 
\draw  [fill={rgb, 255:red, 208; green, 2; blue, 27 }  ,fill opacity=1 ] (85.87,459.53) -- (82.47,465.42) -- (75.67,465.42) -- (72.27,459.53) -- (75.67,453.64) -- (82.47,453.64) -- cycle ;
%Shape: Rectangle [id:dp7608297067867684] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 245; green, 166; blue, 35 }  ,fill opacity=1 ] (207,456.33) -- (238.67,456.33) -- (238.67,459.67) -- (207,459.67) -- cycle ;
%Shape: Rectangle [id:dp8961296544183974] 
\draw  [color={rgb, 255:red, 255; green, 255; blue, 255 }  ,draw opacity=1 ][fill={rgb, 255:red, 0; green, 0; blue, 0 }  ,fill opacity=1 ] (344,458) -- (375.67,458) -- (375.67,461.33) -- (344,461.33) -- cycle ;

% Text Node
\draw (147.63,458.35) node   [align=left] {\begin{minipage}[lt]{74.07pt}\setlength\topsep{0pt}
Graph Node
\end{minipage}};
% Text Node
\draw (290.67,457.83) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
Graph Edge
\end{minipage}};
% Text Node
\draw (429.67,457.5) node   [align=left] {\begin{minipage}[lt]{68pt}\setlength\topsep{0pt}
DG mesh
\end{minipage}};


\end{tikzpicture}


==> P6_2D_Computation_time.tex <==
\subsection{Train, Validation and Test Computation Time}
\seclab{Train_validation_test_computation_time}

In this section, we discuss the computation cost and acceleration benefits of the proposed \oDGNet approaches. The total time for training is the sum of the cost of the training step and validation step. The validation cost is more significant than the training cost. This is because we only solve one time forward for a batch of training samples and update the network with ADAM optimizer, while we have to solve $\frac{T_\text{train}}{\dt}$ time steps during the validation phase from validation initial condition. Ideally, validation should be evaluated at every training epoch, but it is not a mandatory requirement. To decrease the overall training time, we carry out the validation every certain number of epochs, for example, every 200 epochs for the Airfoil problem. This approach might lead to a trade-off where a better network might be missed if the best validation is not coincident with the designated epochs. However, based on our experiment on the Forward Facing Step problem, the best-selected network (validated every epoch) is insignificantly better than the network obtained by sparse validation every 10 epochs. The test time is the total time required to solve the equations for the test data set, either by \oDGNet networks or the traditional DG method. The speed-up rate is the ratio of DG test time to \oDGNet test time. \cref{tab:computational_time} summarizes the training, validation, and test computation time, along with the corresponding speed-up rate of the \oDGNet learning methods, and the GPU hardware used for the Forward Facing Step, Scramjet, Airfoil, Euler Benchmark configuration 6, Double Mach Reflection, and 3D TGV problems. The \mcDGNet converges to the selected network significantly faster than the \nDGNet method for some problems. For instance, the highest convergence rate ratio between the \mcDGNet and \nDGNet method is approximately 54 for the Scramjet problem, while the lowest one is 1.9 for the Double Mach Reflection problem. Note that in this problem the noise-free data is sufficiently informative, thus we expect similar behaviors from both \nDGNet and \mcDGNet approaches in all aspects including training, validation and test accuracy. In comparison with the traditional DG method, we can use pre-trained \mcDGNet networks to solve shock-type problems with a speed-up rate of 5.24, 4.26, 7.61, 3.62, and 3.08 for the Forward Facing Step, Scramjet, Airfoil, Euler Benchmark configuration 6, and Double Mach Reflection problems respectively. It is important to note that the speed-up rate is moderate since the cost of computing the Lax-Friedrichs flux scheme is not expensive. Indeed, in the code implementation, the numerical flux is evaluated using a well-formulated equation, rather than directly solving eigen decomposition problems. Therefore, we anticipate a significant speed-up rate for problems with expensive flux computations. Also, as discussed in \cite{magiera2020constraint}, there are scenarios in particular simulations where the Riemann solver is not available. In that case, the advantages of our \oDGNet approach become clear. Indeed, we can learn surrogate models for the Riemann solver from observation data, and use them to accelerate the computation for other cases.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[htb!]
    \caption{Training, validation and test computation time of \nDGNet and \mcDGNet approaches and the speed improvement compared to traditional DG method for different problems.}
    \tablab{computational_time}
    \begin{tabular}{|cr|ccrr|r|r|r|l|}
        \hline
        \multicolumn{2}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Problems\\ and\\ Approaches\end{tabular}}} &
          \multicolumn{4}{c|}{Training time} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Test\\ (sec)\end{tabular}}} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}DG\\ (sec)\end{tabular}}} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Speed\\ Up\end{tabular}}} &
          \multirow{2}{*}{GPU} \\ \cline{3-6}
        \multicolumn{2}{|c|}{} &
          \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Train \\ (sec\\ /epoch)\end{tabular}} &
          \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Vali-\\ dation \\ (sec)\end{tabular}} &
          \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ Epoch\end{tabular}} &
          \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Total \\ time\\ (hours)\end{tabular}} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{c|}{} &
           \\ \hline
        \multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Forward \\ Facing\end{tabular}}} &
          \nDGNet &
          \multicolumn{1}{c|}{0.006} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}2.07\\ (10$^*$)\end{tabular}}} &
          \multicolumn{1}{r|}{62230} &
          3.68 &
          \multirow{2}{*}{6.45} &
          \multirow{2}{*}{33.85} &
          \multirow{2}{*}{5.24} &
          \multirow{2}{*}{A100} \\ \cline{2-3} \cline{5-6}
        \multicolumn{1}{|c|}{} &
          \mcDGNet &
          \multicolumn{1}{c|}{0.007} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{r|}{1560} &
          0.09 &
           &
           &
           &
           \\ \hline
        \multicolumn{1}{|c|}{\multirow{2}{*}{Scramjet}} &
          \nDGNet &
          \multicolumn{1}{c|}{0.008} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}1.94\\ (10$^*$)\end{tabular}}} &
          \multicolumn{1}{r|}{151200} &
          8.54 &
          \multirow{2}{*}{5.63} &
          \multirow{2}{*}{24.02} &
          \multirow{2}{*}{4.26} &
          \multirow{2}{*}{A100} \\ \cline{2-3} \cline{5-6}
        \multicolumn{1}{|c|}{} &
          \mcDGNet &
          \multicolumn{1}{c|}{0.009} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{r|}{2750} &
          0.16 &
           &
           &
           &
           \\ \hline
        \multicolumn{1}{|c|}{\multirow{2}{*}{Airfoil}} &
          \nDGNet &
          \multicolumn{1}{c|}{0.008} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}2.68\\ (200$^*$)\end{tabular}}} &
          \multicolumn{1}{r|}{1185800} &
          7.09 &
          \multirow{2}{*}{12.70} &
          \multirow{2}{*}{96.65} &
          \multirow{2}{*}{7.61} &
          \multirow{2}{*}{A100} \\ \cline{2-3} \cline{5-6}
        \multicolumn{1}{|c|}{} &
          \mcDGNet &
          \multicolumn{1}{c|}{0.011} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{r|}{472200} &
          3.17 &
           &
           &
           &
           \\ \hline
        \multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Euler\\ Config6\end{tabular}}} &
          \nDGNet &
          \multicolumn{1}{c|}{0.006} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}5.44\\ (500$^*$)\end{tabular}}} &
          \multicolumn{1}{r|}{552500} &
          25.75 &
          \multirow{2}{*}{18.82} &
          \multirow{2}{*}{68.19} &
          \multirow{2}{*}{3.62} &
          \multirow{2}{*}{H100} \\ \cline{2-3} \cline{5-6}
        \multicolumn{1}{|c|}{} &
          \mcDGNet &
          \multicolumn{1}{c|}{0.008} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{r|}{63000} &
          3.30 &
           &
           &
           &
           \\ \hline
        \multicolumn{1}{|c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Double \\ Mach\end{tabular}}} &
          \nDGNet &
          \multicolumn{1}{c|}{0.006} &
          \multicolumn{1}{c|}{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}8.75\\ (100$^*$)\end{tabular}}} &
          \multicolumn{1}{r|}{172500} &
          4.45 &
          \multirow{2}{*}{37.46} &
          \multirow{2}{*}{115.45} &
          \multirow{2}{*}{3.08} &
          \multicolumn{1}{c|}{\multirow{2}{*}{H100}} \\ \cline{2-3} \cline{5-6}
        \multicolumn{1}{|c|}{} &
          \mcDGNet &
          \multicolumn{1}{c|}{0.010} &
          \multicolumn{1}{c|}{} &
          \multicolumn{1}{r|}{73400} &
          2.35 &
           &
           &
           &
          \multicolumn{1}{c|}{} \\ \hline
        % \multicolumn{1}{|c|}{\multirow{2}{*}{3D TGV}} &
        %   \nDGNet &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{c|}{\multirow{2}{*}{}} &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{c|}{\multirow{2}{*}{}} &
        %   \multicolumn{1}{c|}{\multirow{2}{*}{}} &
        %   \multicolumn{1}{l|}{\multirow{2}{*}{}} &
        %   \multirow{2}{*}{} \\ \cline{2-3} \cline{5-6}
        % \multicolumn{1}{|c|}{} &
        %   \mcDGNet &
        %   \multicolumn{1}{l|}{} &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{l|}{} &
        %   \multicolumn{1}{l|}{} &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{c|}{} &
        %   \multicolumn{1}{l|}{} &
        %    \\ \hline
    \end{tabular}
    $^*$ validation is implemented every 10/100/200/500 epochs to reduce the total training time.
\end{table}

% TODO: adding 3D result?



